STSBench: A Spatio-temporal Scenario Benchmark for Multi-modal Large Language Models in Autonomous Driving

We introduce STSBench, a scenario-based framework to benchmark the holistic understanding of vision-language models (VLMs) for autonomous driving. The framework automatically mines pre-defined traffic scenarios from any dataset using ground-truth annotations, provides an intuitive user interface for efficient human verification, and generates multiple-choice questions for model evaluation. Applied to the NuScenes dataset, we present STSnu, the first benchmark that evaluates the spatio-temporal reasoning capabilities of VLMs based on comprehensive 3D perception. Existing benchmarks typically target off-the-shelf or fine-tuned VLMs for images or videos from a single viewpoint and focus on semantic tasks such as object recognition, dense captioning, risk assessment, or scene understanding. In contrast, STSnu evaluates driving expert VLMs for end-to-end driving, operating on videos from multi-view cameras or LiDAR. It specifically assesses their ability to reason about both ego-vehicle actions and complex interactions among traffic participants, a crucial capability for autonomous vehicles. The benchmark features 43 diverse scenarios spanning multiple views and frames, resulting in 971 human-verified multiple-choice questions. A thorough evaluation uncovers critical shortcomings in existing models' ability to reason about fundamental traffic dynamics in complex environments. These findings highlight the urgent need for architectural advances that explicitly model spatio-temporal reasoning. By addressing a core gap in spatio-temporal evaluation, STSBench enables the development of more robust and explainable VLMs for autonomous driving.

==> _preamble.tex <==
\RequirePackage{xspace}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{graphicx}

\usepackage{amssymb}%
\usepackage{pifont}%

\usepackage{array}
\usepackage{tabularx}
\usepackage[table]{xcolor}

\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usepackage{sansmath}
\usepackage{rotating} %
\usetikzlibrary{pgfplots.statistics}
\usetikzlibrary{intersections}
\usepgfplotslibrary{fillbetween}
\usepackage{pgfplotstable}
\usetikzlibrary{pie}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage[most]{tcolorbox}
\usepackage{wrapfig}
\usetikzlibrary{matrix, positioning, fit}
\usepackage{fontawesome5}
\usepackage{adjustbox}
\usepackage[normalem]{ulem}

\usepackage[toc,page,header]{appendix}
\usepackage{minitoc}  

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newcommand{\ourBenchmark}{STSBench\xspace}
\newcommand{\ourBenchmarkNus}{STSnu\xspace}
\newcommand{\ourBenchmarkUrl}{STSBench3D}
\newcommand{\nScenarios}{43\xspace}
\newcommand{\nScenariosTotal}{4790\xspace}
\newcommand{\nScenariosSampled}{1188\xspace}
\newcommand{\nQuestions}{971\xspace}

\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\rewrite}[1]{{\color{orange}#1}}
\newcommand{\opt}[1]{\textcolor[rgb]{0.0, 0.372, 0.416}{\textbf{#1}}}
\newcommand{\cfr}[1]{\textcolor[rgb]{0.2, 0.537, 0.62}{\textbf{CFR: #1}}}

\newcommand{\mrrot}[2]{\multirow{#1}{*}{\rotatebox[origin=c]{90}{#2}}}
\newcommand{\mr}[2]{\multirow{#1}{*}{{#2}}}



\input{abbreviations}


\definecolor{C0}{HTML}{1F77B4}
\definecolor{C1}{HTML}{FF7F0E}
\definecolor{C2}{HTML}{2CA02C}
\definecolor{C3}{HTML}{d62728}
\definecolor{C4}{HTML}{9467BD}
\definecolor{C5}{HTML}{8c564b}
\definecolor{C6}{HTML}{e377c2}
\definecolor{C7}{HTML}{7f7f7f}
\definecolor{C8}{HTML}{bcbd22}
\definecolor{C9}{HTML}{17becf}

\definecolor{PromptGray}{HTML}{f2f2f2}
\definecolor{PromptBorder}{HTML}{231f20}

\tikzstyle{PromptBox} = [draw=PromptBorder, fill=PromptGray!100, very thick,
    rectangle, rounded corners, inner sep=10pt, inner ysep=20pt]
\tikzstyle{PromptTitle} =[fill=PromptBorder, text=white]

\tikzstyle{SystemPromptBox} = [draw=C0, fill=c0!70, very thick,
    rectangle, rounded corners, inner sep=10pt, inner ysep=20pt]
\tikzstyle{SystemPromptTitle} =[fill=C0, text=white]

\renewcommand \thepart{}
\renewcommand \partname{}




==> abbreviations.tex <==
\newcommand{\lidar}{LiDAR\xspace}
\newcommand{\nus}{NuScenes\xspace}
\newcommand{\kitti}{KITTI\xspace}
\newcommand{\once}{ONCE\xspace}
\newcommand{\wod}{WOD\xspace}
\newcommand{\carla}{CARLA\xspace}

\newcommand{\covla}{CoVLA~\cite{arai_2024_covla}\xspace}
\newcommand{\maplm}{MAPLM~\cite{cao_2024_maplm}\xspace}
\newcommand{\drivemllm}{DriveMLLM~\cite{guo_2024_drivemllm}\xspace}
\newcommand{\nuscenesmqa}{\nus-MQA~\cite{inoue_2024_nuscenes_mqa}\xspace}
\newcommand{\vladbench}{VLADBench~\cite{li_2025_vladbench}\xspace}
\newcommand{\lingoqa}{LingoQA~\cite{marcu_2024_lingoqa}\xspace}
\newcommand{\reasontodrive}{Reason2Drive~\cite{nie_2023_reason2drive}\xspace}
\newcommand{\ranktotell}{Rank2Tell~\cite{sachdeva_2024_rank2tell}\xspace}
\newcommand{\nuscenesqa}{\nus-QA~\cite{qian_2024_nuscenesqa}\xspace}
\newcommand{\drivelm}{DriveLM~\cite{sima_2024_drivelm}\xspace}
\newcommand{\evalllmdrive}{EVAL\_LLM\_DRIVE~\cite{sreeram_2024_probing}\xspace}
\newcommand{\nuscenesspatialqa}{\nus-SpatialQA~\cite{tian_2025_nuscenesspatialqa}\xspace}
\newcommand{\metavqa}{Meta-VQA~\cite{wang_2025_metavqa}\xspace}
\newcommand{\drivebench}{DriveBench~\cite{xie_2025_drivebench}\xspace}
\newcommand{\dvbench}{DVBench~\cite{zeng_2025_dvbench}\xspace}
\newcommand{\nuinstruct}{NuInstruct~\cite{ding_2024_holistic}\xspace}
\newcommand{\todcap}{TOD3Cap~\cite{jin_2024_tod3cap}\xspace}
\newcommand{\drivelmmoone}{DriveLLM-o1~\cite{ishaq_2025_drivelmmo1}\xspace}
\newcommand{\codalm}{CODA-LM~\cite{li_2024_codalm}\xspace} %
\newcommand{\drama}{DRAMA~\cite{malla_2023_drama}\xspace}
\newcommand{\nuplanqa}{NuPlanQA~\cite{park_2025_nuplanqa}\xspace}
\newcommand{\sennads}{DriveX~\cite{jiang_2024_senna}\xspace}
\newcommand{\wodc}{\wod~\cite{sun_2020_waymo}\xspace}
\newcommand{\kittic}{\kitti~\cite{geiger_2012_kitti}\xspace}
\newcommand{\oncec}{\once~\cite{mao_2021_once}\xspace}
\newcommand{\nusc}{\nus~\cite{caesar_2020_nuscenes}\xspace}
\newcommand{\carlac}{\carla~\cite{dosovitskiy_2017_carla}\xspace}
\newcommand{\nd}{New dataset\xspace}
\newcommand{\rtdc}{Mult.~\cite{caesar_2020_nuscenes, mao_2021_once, sun_2020_waymo}\xspace}
\newcommand{\codac}{Mult.~\cite{caesar_2020_nuscenes, geiger_2012_kitti, mao_2021_once}\xspace}

\newcommand{\orion}{ORION~\cite{fu_2025_orion}\xspace}
\newcommand{\bevinmllm}{BEV-InMLLM~\cite{ding_2024_holistic}\xspace}
\newcommand{\emma}{EMMA~\cite{hwang_2024_emma}\xspace}
\newcommand{\sennavlm}{Senna-VLM~\cite{jiang_2024_senna}\xspace}
\newcommand{\gpvl}{GPVL~\cite{li_2025_gpvl}\xspace}
\newcommand{\vlp}{VLP~\cite{pan_2024_vlp}\xspace}
\newcommand{\lmdrive}{LMDrive~\cite{shao_2024_lmdrive}\xspace}
\newcommand{\insightdrive}{InsightDrive~\cite{song_2025_insightdrive}\xspace}
\newcommand{\omnidrive}{OmniDrive~\cite{wang_2024_omnidrive}\xspace}
\newcommand{\scetwodrivex}{Sce2DriveX~\cite{zhao_2025_sce2drivex}\xspace}
\newcommand{\opendrivevla}{OpenDriveVLA~\cite{zhou_2025_opendrivevla}\xspace}
\newcommand{\hermes}{HERMES~\cite{zhou_2025_hermes}\xspace}
\newcommand{\bevdriver}{BEVDriver~\cite{winter_2025_bevdriver}\xspace}
\newcommand{\drivevlmdual}{DriveVLM-Dual~\cite{sima_2024_drivelm}\xspace}
\newcommand{\rdadriver}{RDA-Driver~\cite{huang_2024_rdadriver}\xspace}
\newcommand{\drivemm}{DriveMM~\cite{huang_2024_drivemm}\xspace}

\newcommand{\quenvlsb}{Qwen2.5-VL~7B~\cite{shuai_2025_quenvl}\xspace}
\newcommand{\internvlab}{InternVL~2.5~8B~\cite{chen_2024_internvl}\xspace}
\newcommand{\internvlob}{InternVL~2.5~1B~\cite{chen_2024_internvl}\xspace}

\newcommand{\gptfo}{GPT-4o~\cite{openai_2024_gpt4}\xspace}
\newcommand{\deepseek}{DeepSeek~V3~\cite{deepseekai_2024_deepseekv3}\xspace}
\newcommand{\llama}{Llama~3.2~\cite{meta_2025_llama3}\xspace}

\newcommand{\bestresult}[1]{\text{\textbf{#1}}}
\newcommand{\secbresult}[1]{\underline{#1}}





